IMELL Cut Elimination with Linear Overhead

Recently, Accattoli introduced the Exponential Substitution Calculus (ESC) given by untyped proof terms for Intuitionistic Multiplicative Exponential Linear Logic (IMELL), endowed with rewriting rules at-a-distance for cut elimination. He also introduced a new cut elimination strategy, dubbed the good strategy, and showed that its number of steps is a time cost model with polynomial overhead for the ESC/IMELL, and the first such one. Here, we refine Accattoli's result by introducing an abstract machine for ESC and proving that it implements the good strategy and computes cut-free terms/proofs within a linear overhead.

==> 08-Conclusions.tex <==
% !TEX root = main.tex
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\section{Conclusions}
%\section{Exponential Exploding Family}
%Example: $\cuta{\bang\bang\la\evar\dera\evar\evartwo}{\evar_3}
%\cuta{\bang \dera{\evar_3}{\_} \dera{\evar_3}{\evartwo_3} \evartwo_3 }{\evar_2}
%\cuta{\bang \dera{\evar_2}{\_} \dera{\evar_2}{\evartwo_2} \evartwo_2 }{\evar_1}
%\cuta{\bang \dera{\evar_1}{\_} \dera{\evar_1}{\evartwo_1} \evartwo_1 }{\evar_0}
%\dera{\evar_0}{\evartwo_0} \evartwo_0$.\medskip
%
%Definition of the n-th term $\tmtwo_n$ of the family:
%\begin{itemize}
%\item $\tm_0 \defeq \dera{\evar_0}{\evartwo_0} \evartwo_0$.
%\item $\tm_{n+1} \defeq \cuta{\bang \dera{\evar_{n+1}}{\_} \dera{\evar_{n+1}}{\evartwo_{n+1}} \evartwo_{n+1} }{\evar_n} \tm_n$.
%\item $\tmtwo_n \defeq \cuta{\bang\bang\la\evar\dera\evar\evartwo}{\evar_n}\tm_n$.
%\end{itemize}
%
%\subsection{For the SCOT talk}
%Definition of the n-th term $\tmtwo_n$ of the family:
%\begin{itemize}
%\item $\tm_0 \defeq \dera{\evar_{0}}{\_}\dera{\evar_0}{\evartwo_0} \evartwo_0$.
%\item $\tm_{n+1} \defeq \cuta{\bang \dera{\evar_{n+1}}{\_} \dera{\evar_{n+1}}{\evartwo_{n+1}} \evartwo_{n+1} }{\evar_n} \tm_n$.
%\item $\tmtwo_n \defeq \cuta{\bang\bang\la\evar\dera\evar\evartwo}{\evar_n}\tm_n$.
%\end{itemize}
%
%\[\begin{array}{lllllllllll}
%\tm_1 & = & \cuta{\bang \dera{\evar_{1}}{\_} \dera{\evar_{1}}{\evartwo_{1}} \evartwo_{1} }{\evar_0} & \dera{\evar_{0}}{\_}\dera{\evar_0}{\evartwo_0} \evartwo_0
%\\
%&\tobang&
%\cuta{\bang \dera{\evar_{1}}{\_} \dera{\evar_{1}}{\evartwo_{1}} \evartwo_{1} }{\evar_0} & \dera{\evar_{1}}{\_} \dera{\evar_{1}}{\evartwo_{1}'} \cuta{\evartwo_{1}'}{\_} \dera{\evar_0}{\evartwo_0} \evartwo_0
%\\
%&\tobang&
%\cuta{\bang \dera{\evar_{1}}{\_} \dera{\evar_{1}}{\evartwo_{1}} \evartwo_{1} }{\evar_0} & \dera{\evar_{1}}{\_} \dera{\evar_{1}}{\evartwo_{1}'} \cuta{\evartwo_{1}'}{\_} \dera{\evar_{1}}{\_} \dera{\evar_{1}}{\evartwo_{1}''} \cuta{\evartwo_{1}''}{\evartwo_0} \evartwo_0
%
%\end{array}\]

==> machines/closed_machine_implicit.tex <==
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
  \begin{tabular}{c}
  $\begin{array}{r\colspace rcl\colspace|\colspace r\colspace rclll}
%  \multicolumn{8}{c}{\textsc{Data structures, States, and Initialization}}
%  \\[3pt]
%
%  \textsc{Environments} & \ectx,\ectxtwo & \grameq & \eempty \mid \ectx\cuta\val\var
  
    \textsc{States} & \state,\statetwo & \grameq & \twostate\ectx\tm
    &
  \textsc{Initialization} & \compilrel\tm\state & \mbox{if} & \state=\twostate\ctxhole{\rename\tm}
  \\
  \textsc{Read back} & \decode{\twostate\ectx\tm} & \defeq & \ectx\ctxholep\tm
    \end{array}$
%%%%%%%%%%%
    \\[18pt]
%%%%%%%%%%%
$\begin{array}{r@{\hspace{.2cm}}|@{\hspace{.2cm}}r@{\hspace{.2cm}}||@{\hspace{.2cm}}l@{\hspace{.2cm}}||@{\hspace{.2cm}}r@{\hspace{.2cm}}|@{\hspace{.2cm}}r}
      \multicolumn{5}{c}{\textsc{Transitions}}
      \\[3pt]
\textsc{Cut Ctx} & \textsc{Active Tm} & & \textsc{Cut Ctx} & \textsc{Active Tm}
\\\hline\hline
\ectx & \cuta\val\var \tm
&\tomachsea&
\ectxp{\cuta\val\var\ctxhole} &\tm
\\[4pt]

%\ectx   \cuta{\mvartwo}\mvar   \ectxtwo & \para\mvar\var\vartwo\tm
%&\tomachaxmone&
%\ectx   \ectxtwo & \para\mvartwo\var\vartwo\tm
%\\

\ectxp{   \cuta{\mvartwo}\mvar   \ectxtwo} & \suba\mvar\val\var\tm
&\tomachaxmtwo&
\ectxp   \ectxtwo & \suba\mvartwo\val\var\tm
\\

%\ectx   \cuta{\tensa{\lctxp\val}{\ectxtwop\valtwo}}\mvar   \ectxtwo & \para\mvar\var\vartwo \tm
%&\tomachtens&
%\ectx   \ectxtwo &\lctxp{\cuta\val\var\ectxtwop{\cuta\valtwo\vartwo\tm}}
%\\

\ectxp{   \cuta{\la\vartwo\lctxp\valtwo}\mvar   \ectxtwo} & \suba\mvar\val\var \tm
&\tomachlolli&
\ectxp{  \ectxtwo  \cuta\val\vartwo } &\lctxp{\cuta\valtwo\var\tm}
\\

\ectxp{   \cuta{\evartwo}\evar   \ectxtwo} & \dera\evar\var\tm
&\tomachaxetwo&
\ectxp{   \cuta{\evartwo}\evar   \ectxtwo} & \dera\evartwo\var\tm
\\

\ectxp{   \cuta{\bang\lctxp\val}\evar   \ectxtwo} & \dera\evar\var\tm
&\tomachbang&
\ectxp{   \cuta{\bang\lctxp\val}\evar   \ectxtwo} & \rename\lctx\ctxholep{\cuta{\rename\val}\var\tm}
\\[4pt]

\ectxp{   \cuta{\mval}\mvar   \ectxtwo} & \mvar
&\tomachaxmone&
\ectxp   \ectxtwo &\mval
\\

\ectxp{   \cuta{\exval}\evar   \ectxtwo} & \evar
&\tomachaxeone&
\ectxp{   \cuta{\exval}\evar   \ectxtwo} &\rename\exval\\
\end{array}$
%%%%%%%%%%%
%    \\[56pt]
%%%%%%%%%%%%
%      $\begin{array}{rll\colspace\colspace rll}
%  \multicolumn{6}{c}{\textsc{Read back}}
%  \\[3pt]
%  \decode{\twostate\eempty\tm} & \defeq & \tm
%  &
%  \decode{\twostate{\ectx\cuta\val\var}\tm} & \defeq & \decode{\twostate{\ectx}{\cuta\val\var\tm}}
%    \end{array}$
\end{tabular}

==> machines/garbage_collector.tex <==
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
$\begin{array}{r|r||@{\hspace{.2cm}}l@{\hspace{.2cm}}||r|r}
\textsc{Appr.} & \textsc{Pool} && \textsc{Appr.} & \textsc{Pool}
\\\hline\hline
\namctx & \nctxholep{\cuta\val\var \tm}\name \cons \pool 
&\tomachgcw&
\namctx &\nctxholep{\tm}\name \cons \pool
\\
\namctx & \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool  
&\tomachgcseatwo&
\namctx  \nctxholep{\suba\mvar{\nctxhole\nametwo}\var \nctxhole\name}\name &\nctxholep{\val}\nametwo \cons \nctxholep{\tm}\name  \cons\pool
\\
\namctx & \nctxholep{\dera\evar\var\tm}\name \cons \pool
&\tomachgcseathree&
\namctx   \nctxholep{\dera\evar\var \nctxhole\name}\name &\nctxholep{\tm}\name \cons \pool
\\
\namctx    & \nctxholep{\la\var\tm}\name \cons \pool  
&\tomachgcseafour&
\namctx  \nctxholep{ \la\var\nctxhole\name}\name &\nctxholep{\tm}\name \cons \pool
\\
\namctx    & \nctxholep{\bang\tm}\name \cons \pool  
&\tomachgcseafive&
\namctx  \nctxholep{ \bang\nctxhole\name}\name &\nctxholep{\tm}\name \cons \pool
\\
\namctx   & \nctxholep{\var}\name  \cons \pool  
&\tomachgcseasix&
\namctx  \nctxholep\var\name &\pool
\end{array}$

==> machines/strong_machine_implicit.tex <==
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
  \begin{tabular}{c}
  $\begin{array}{r\colspace rcl\colspace|\colspace r\colspace rclll}
%  \multicolumn{8}{c}{\textsc{Data structures, States, and Initialization}}
%  \\[3pt]
%
%  \textsc{Environments} & \ectx,\ectxtwo & \grameq & \eempty \mid \ectx\cuta\val\var
  
    \textsc{Pools} & \pool,\pooltwo & \grameq & \emptylist \mid \namctxholep\tm\name \cons \pool
    &
  \textsc{Init.} & \compilrel\tm\state & \mbox{if} & \state=\twostate\namctxholea{\rename\tm}
    \\
    \textsc{States} & \state,\statetwo & \grameq & \twostate\namctx\pool
  &
  \textsc{Read back} & \decode{\twostate\namctx\pool} & \defeq & \namctx\namctxholep{\tm_1}{\name_1}\ldots\namctxholep{\tm_k}{\name_k}
  \\
  &&&&&\multicolumn{3}{r}{\mbox{with }\pool=\namctxholep{\tm_1}{\name_1}\cons\ldots\cons\namctxholep{\tm_k}{\name_k}}
    \end{array}$
%%%%%%%%%%%
    \\[18pt]
$\begin{array}{r|r||@{\hspace{.2cm}}l@{\hspace{.2cm}}||r|r|ll}
\textsc{MCtx} & \textsc{Pool} && \textsc{MCtx} & \textsc{Pool}
\\\hline\hline
\twostatetranstab \namctx { \nctxholep{\cuta\val\var \tm}\name \cons \pool }
\tomachseaone
{ \namctxp{\cuta\val\var \nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
\\
\twostatetranstab \namctx { \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool }
\tomachseatwo
{ \namctx\nctxholep{\suba\mvar{\nctxhole\nametwo}\var \nctxhole\name}\name } { \nctxholep{\val}\nametwo \cons \nctxholep{\tm}\name  \cons\pool }
&\mbox{if }\mvar\notin\domp\namctx, $\nametwo$ \mbox{ fresh}
\\
\twostatetranstab \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachseathree
{ \namctx\nctxholep{\dera\evar\var \nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
&\mbox{if }\evar\notin\domp\namctx
\\
\twostatetranstab \namctx { \nctxholep{\la\var\tm}\name \cons \pool }
\tomachseafour
{ \namctxp{ \la\var\nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
\\
\twostatetranstab \namctx  { \nctxholep{\bang\tm}\name \cons \pool }
\tomachseafive
{ \namctxp{\bang\nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
\\
\twostatetranstab \namctx { \nctxholep{\var}\name \cons \pool }
\tomachseasix
{ \namctxp\var\name } \pool
&\mbox{if }\var\notin\domp\namctx

\\[4pt]
\hline
%\namctx   \cuta{\mvartwo}\mvar   \namctxtwo & \para\mvar\var\vartwo\tm
%&\toaxmone&
%\namctx   \namctxtwo & \para\mvartwo\var\vartwo\tm
%\\

\twostatetranstab \namctx { \nctxholep{\suba\mvar\val\var\tm}\name \cons \pool }
\tomachaxmtwo
{ \namctx\setminus\mvar } { \nctxholep{\suba\mvartwo\val\var\tm}\name \cons \pool }
&\mbox{if }\namctx(\mvar)=\mvartwo
\\

%\namctx   \cuta{\tensa{\namctxp\val}{\namctxtwop\valtwo}}\mvar   \namctxtwo & \para\mvar\var\vartwo \tm
%&\totens&
%\namctx   \namctxtwo &\namctxp{\cuta\val\var\namctxtwop{\cuta\valtwo\vartwo\tm}}
%\\

\twostatetranstab \namctx { \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool }
\tomachlolli
{ \namctx\setminus\mvar } { \nctxholep{\cuta\val\vartwo\lctxp{\cuta\valtwo\var\tm}}\name \cons \pool }
&\mbox{if }\namctx(\mvar)=\la\vartwo\lctxp\valtwo
\\

\twostatetranstab \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachaxetwo
\namctx { \nctxholep{\dera\evartwo\var\tm}\name \cons \pool }
&\mbox{if }\namctx(\evar)=\evartwo
\\

\twostatetranstab \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachbang
\namctx { \nctxholep{\rename\lctx\ctxholep{\cuta{\rename\val}\var\tm}}\name \cons \pool }
&\mbox{if }\namctx(\evar)=\bang\lctxp\val
\\

\twostatetranstab \namctx { \nctxholep{\mvar}\name \cons \pool }
\tomachaxmone
{ \namctx\setminus \mvar } { \nctxholep{\mval}\name \cons \pool }
&\mbox{if }\namctx(\mvar)=\mval
\\

\twostatetranstab \namctx { \nctxholep{\evar}\name \cons \pool }
\tomachaxeone
\namctx { \nctxholep{\exval}\name \cons \pool }
&\mbox{if }\namctx(\evar)=\exval
\end{array}$
\end{tabular}

==> proofs/invariants-blueprint-explicit.tex <==
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\begin{itemize}
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\cuta\val\var \tm}\name \cons \pool } 
\tomachseaone
{ \namctx  \nctxholep{\cuta\val\var \nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }=\state$.

% SEA 2
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool }
\tomachseatwo
{ \namctx\nctxholep{\suba\mvar{\nctxhole\nametwo}\var \nctxhole\name}\name } { \nctxholep{\val}\nametwo \cons \nctxholep{\tm}\name  \cons\pool } =\state$ if $\mvar\notin\domp\namctx$ and $\nametwo$ is fresh.

% SEA 3
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachseathree
 { \namctx   \nctxholep{\dera\evar\var \nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
 =\state$  if $\evar\notin\domp\namctx$.

% SEA 4
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\la\var\tm}\name \cons \pool  }
\tomachseafour
{ \namctx  \nctxholep{ \la\var\nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
 =\state$.

% SEA 5
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\bang\tm}\name \cons \pool  }
\tomachseafive
{ \namctx  \nctxholep{ \bang\nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
 =\state$.

% SEA 6
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\var}\name  \cons \pool }
\tomachseasix
{ \namctx  \nctxholep\var\name }\pool
 =\state$  if $\var\notin\domp\namctx$.

% AX M 2
\item $\statetwo = \twostatetrans { \namctxp{\cuta\mvartwo\mvar\namctxtwo}\mute } { \nctxholep{\suba\mvar\val\var\tm}\name \cons \pool }
\tomachaxmtwo
{ \namctxp\namctxtwo\mute } { \nctxholep{\suba\mvartwo\val\var\tm}\name \cons \pool } = \state$.

% LOLLI
\item $\statetwo = \twostatetrans { \namctxp{\cuta{\la\vartwo\lctxp\valtwo}\mvar\namctxtwo}\mute } { \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool }
\tomachlolli
{ \namctxp\namctxtwo\mute } { \nctxholep{\cuta\val\vartwo\lctxp{\cuta\valtwo\var\tm}}\name \cons \pool } = \state$.

% AX E 2
\item $\statetwo = \twostatetrans { \namctxp{\cuta\evartwo\evar\namctxtwo}\mute } { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachaxetwo
{ \namctxp{\cuta\evartwo\evar\namctxtwo}\mute } { \nctxholep{\dera\evartwo\var\tm}\name \cons \pool } = \state$.

% BANG
\item $\statetwo = \twostatetrans { \namctxp{\cuta{\bang\lctxp\val}\evar\namctxtwo}\mute } { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachbang
{ \namctxp{\cuta{\bang\lctxp\val}\evar\namctxtwo}\mute } { \nctxholep{\rename\lctx\ctxholep{\cuta{\rename\val}\var\tm}}\name \cons \pool } = \state$.

% AX M 1
\item $\statetwo = \twostatetrans { \namctxp{\cuta\mval\mvar\namctxtwo}\mute } { \nctxholep{\mvar}\name \cons \pool }
\tomachaxmone
{ \namctxp\namctxtwo\mute } { \nctxholep{\mval}\name \cons \pool } = \state$.

% AX E 1
\item $\statetwo = \twostatetrans { \namctxp{\cuta\exval\evar\namctxtwo}\mute } { \nctxholep{\evar}\name \cons \pool }
\tomachaxeone
{ \namctxp{\cuta\exval\evar\namctxtwo}\mute } { \nctxholep{\exval}\name \cons \pool } = \state$.
\end{itemize}

==> proofs/invariants-blueprint-implicit.tex <==
% !TEX root = ../main.tex
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\begin{itemize}
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\cuta\val\var \tm}\name \cons \pool } 
\tomachseaone
{ \namctx  \nctxholep{\cuta\val\var \nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }=\state$

% SEA 2
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool }
\tomachseatwo
{ \namctx\nctxholep{\suba\mvar{\nctxhole\nametwo}\var \nctxhole\name}\name } { \nctxholep{\val}\nametwo \cons \nctxholep{\tm}\name  \cons\pool } =\state$ if $\mvar\notin\cdom\namctx$ and $\nametwo$ is fresh.

% SEA 3
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachseathree
 { \namctx   \nctxholep{\dera\evar\var \nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
 =\state$  if $\evar\notin\cdom\namctx$.

% SEA 4
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\la\var\tm}\name \cons \pool  }
\tomachseafour
{ \namctx  \nctxholep{ \la\var\nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
 =\state$.

% SEA 5
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\bang\tm}\name \cons \pool  }
\tomachseafive
{ \namctx  \nctxholep{ \bang\nctxhole\name}\name } { \nctxholep{\tm}\name \cons \pool }
 =\state$.

% SEA 6
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\var}\name  \cons \pool }
\tomachseasix
{ \namctx  \nctxholep\var\name }\pool
 =\state$  if $\var\notin\cdom\namctx$.

% AX M 2
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\suba\mvar\val\var\tm}\name \cons \pool }
\tomachaxmtwo
{ \namctx\setminus\mvar } { \nctxholep{\suba\mvartwo\val\var\tm}\name \cons \pool } = \state$
if $\namctx(\mvar)=\mvartwo$.

% LOLLI
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\suba\mvar\val\var \tm}\name \cons \pool }
\tomachlolli
{ \namctx\setminus\mvar } { \nctxholep{\cuta\val\vartwo\lctxp{\cuta\valtwo\var\tm}}\name \cons \pool } = \state$
if $\namctx(\mvar)=\la\vartwo\lctxp\valtwo$.

% AX E 2
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachaxetwo
\namctx { \nctxholep{\dera\evartwo\var\tm}\name \cons \pool } = \state$
if $\namctx(\evar)=\evartwo$.

% BANG
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\dera\evar\var\tm}\name \cons \pool }
\tomachbang
\namctx { \nctxholep{\rename\lctx\ctxholep{\cuta{\rename\val}\var\tm}}\name \cons \pool } = \state$
if $\namctx(\evar)=\bang\lctxp\val$.

% AX M 1
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\mvar}\name \cons \pool }
\tomachaxmone
{ \namctx\setminus \mvar } { \nctxholep{\mval}\name \cons \pool } = \state$
if $\namctx(\mvar)=\mval$.

% AX E 1
\item $\statetwo = \twostatetrans \namctx { \nctxholep{\evar}\name \cons \pool }
\tomachaxeone
\namctx { \nctxholep{\exval}\name \cons \pool } = \state$
if $\namctx(\evar)=\exval$.
\end{itemize}
